VHM: Versatile and Honest Vision Language Model for Remote Sensing Image Analysis

This paper develops a Versatile and Honest vision language Model (VHM) for remote sensing image analysis. VHM is built on a large-scale remote sensing image-text dataset with rich-content captions (VersaD), and an honest instruction dataset comprising both factual and deceptive questions (HnstD). Unlike prevailing remote sensing image-text datasets, in which image captions focus on a few prominent objects and their relationships, VersaD captions provide detailed information about image properties, object attributes, and the overall scene. This comprehensive captioning enables VHM to thoroughly understand remote sensing images and perform diverse remote sensing tasks. Moreover, different from existing remote sensing instruction datasets that only include factual questions, HnstD contains additional deceptive questions stemming from the non-existence of objects. This feature prevents VHM from producing affirmative answers to nonsense queries, thereby ensuring its honesty. In our experiments, VHM significantly outperforms various vision language models on common tasks of scene classification, visual question answering, and visual grounding. Additionally, VHM achieves competent performance on several unexplored tasks, such as building vectorizing, multi-label classification and honest question answering. We will release the code, data and model weights at https://github.com/opendatalab/VHM .

==> table/RAIT_data_construction.tex <==
\begin{algorithm}[t]
\caption{RAIT Data Construction Process}
\label{alg:RAI_data}
\textbf{Input:}{~$D_{\text{src}} = \{x_{0}, x_{1}, ..., x_{N}\}$}, $\tau_\mu$, $N_{\text{van}}$, $N_{\text{idk}}$ \\
\textbf{Output:}{~$D_{rait}\subseteq D_{\text{src}}$}
\begin{algorithmic}[1]
\fontsize{9}{8}
\State $D_{\text{van}}^1 = \{x_i \, | \, x_i \in D_{\text{src}},  x_i.\mu \geq \tau_\mu\}$
\State $D_{\text{idk}}^1 = \{x_j \, | \, x_j \in D_{\text{src}}, x_j.\mu < \tau_\mu \text{ and } x_j.\Delta\mu < 0\}$
\State $D_{\text{\text{van}}}^1 = \text{sort}(D_{\text{van}}^1, \text{key}=\sigma, \text{order=descend})$
\State $D_{\text{idk}}^1 = \text{sort}(D_{\text{idk}}^1, \text{key}=\sigma, \text{order=ascend})$
\State $D_{\text{van}}^2 = \text{TopK}(D_{\text{van}}^1, N_{\text{van}})$
\State $D_{\text{idk}}^2 = \text{TopK}(D_{\text{idk}}^1, N_{\text{idk}})$
\For{$x_i$ in $D_{\text{van}}^2$}
    \State $x_i.a_{\text{rait}}$ = $x_i.a$
\EndFor
\For{$x_j$ in $D_{\text{idk}}^2$}
    \State $x_j.a_{\text{rait}}$ = ``I don't know"
\EndFor
\State $D_{\text{rait}} = D_{\text{van}}^2 \cup D_{\text{idk}}^2$
\State \textbf{return} $D_{\text{rait}}$
\end{algorithmic}
\end{algorithm}



==> table/ab_MCQA_Rehearsal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|lll|lll|}
\hline
\multicolumn{1}{|l|}{}          & \textbf{}             & \multicolumn{3}{c|}{\textbf{MMLU (ID)}}                                                                       & \multicolumn{3}{c|}{\textbf{ARC-c (OOD)}}                                                                     \\ \hline
\textbf{Method}                 & \textbf{$n_{\text{rhs}}$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\textbf{Init-Basic}             & \textbf{-}            & \multicolumn{1}{l|}{66.9}           & \multicolumn{1}{l|}{33.1}           & 0                                 & \multicolumn{1}{l|}{80.6}           & \multicolumn{1}{l|}{19.5}           & 0                                 \\ \hline
\textbf{Init-Refuse}            & \textbf{-}            & \multicolumn{1}{l|}{50}             & \multicolumn{1}{l|}{17}             & 15.6                              & \multicolumn{1}{l|}{65.3}           & \multicolumn{1}{l|}{14.4}           & 5.6                               \\ \hline
\textbf{Van-Tuning}             & \textbf{-}            & \multicolumn{1}{l|}{69.5}           & \multicolumn{1}{l|}{30.5}           & 8                                 & \multicolumn{1}{l|}{80.3}           & \multicolumn{1}{l|}{19.7}           & -1.3                              \\ \hline
\textbf{Cor-RAIT}               & \textbf{-}            & \multicolumn{1}{l|}{63.9}           & \multicolumn{1}{l|}{21.6}           & 20.4                              & \multicolumn{1}{l|}{66.8}           & \multicolumn{1}{l|}{16.2}           & 12.2                              \\ \hline
\multirow{4}{*}{\textbf{CRaFT}} & \textbf{200}          & \multicolumn{1}{l|}{54.1}           & \multicolumn{1}{l|}{12.2}           & 27.7                              & \multicolumn{1}{l|}{74.5}           & \multicolumn{1}{l|}{14.2}           & 15.9                              \\ \cline{2-8} 
                                & \textbf{500}          & \multicolumn{1}{l|}{55.8}           & \multicolumn{1}{l|}{13.6}           & 28.4                              & \multicolumn{1}{l|}{76}             & \multicolumn{1}{l|}{15}             & 13.8                              \\ \cline{2-8} 
                                & \textbf{1000}         & \multicolumn{1}{l|}{53.3}           & \multicolumn{1}{l|}{9.6}            & 34                                & \multicolumn{1}{l|}{74.1}           & \multicolumn{1}{l|}{12.7}           & 21.4                              \\ \cline{2-8} 
                                & \textbf{1629}    & \multicolumn{1}{l|}{54.7}           & \multicolumn{1}{l|}{11.4}           & 31.2                              & \multicolumn{1}{l|}{75}             & \multicolumn{1}{l|}{14.8}           & 13.9                              \\ \hline
\end{tabular}
{\fontsize{9pt}{11pt}\selectfont
\caption{Results of Reheasal Training in MCQA Task ($\mathcal{M}_{0}$ is LLaMA3-8B-Instruct).}
\label{table:ab_MCQA_rehearsal}}
\end{table}
\endgroup  % End the group

==> table/ab_MCQA_llama2.tex <==
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}

\begin{table}[t]
\centering
{\fontsize{9pt}{11pt}\selectfont
\label{table:ab_exp_MCQA}
\begin{tabular}{|c|ll|ll|}
\hline
\multicolumn{1}{|l|}{}  & \multicolumn{2}{c|}{\textbf{MMLU (ID)}}                                 & \multicolumn{2}{c|}{\textbf{ARC-c (OOD)}}                               \\ \hline
\textbf{Method}         & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\textbf{Cor-RAIT}       & \multicolumn{1}{l|}{39.57}          & 11.32                             & \multicolumn{1}{l|}{38.14}          & 11.08                             \\ \hline
\textbf{CRaFT w/o Flow} & \multicolumn{1}{l|}{31.01}         & 12.97                             & \multicolumn{1}{l|}{32.34}          & 13.45                             \\ \hline
\textbf{CRaFT w/o Cer}  & \multicolumn{1}{l|}{32.05}          & 11.51                             & \multicolumn{1}{l|}{32.94}          & 13.85                             \\ \hline
\textbf{CRaFT}          & \multicolumn{1}{l|}{36.39}          & 12.46                             & \multicolumn{1}{l|}{35.92}          & 12.58                             \\ \hline
\end{tabular}
}
\caption{Ablation Experiment Results in MCQA Task}
\vspace{-10pt}
\end{table}
\endgroup  % End the group

==> table/ab_OEQA_Rehearsal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|lll|lll|}
\hline
\multicolumn{1}{|l|}{}          & \textbf{}             & \multicolumn{3}{c|}{\textbf{TriviaQA (ID)}}                                                                   & \multicolumn{3}{c|}{\textbf{NQ (OOD)}}                                                                        \\ \hline
\textbf{Method}                 & \textbf{$n_{\text{rhs}}$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\textbf{Init-Basic}             & \textbf{-}            & \multicolumn{1}{l|}{54}             & \multicolumn{1}{l|}{46}             & 0                                 & \multicolumn{1}{l|}{29.3}           & \multicolumn{1}{l|}{70.7}           & 0                                 \\ \hline
\textbf{Init-Refuse}            & \textbf{-}            & \multicolumn{1}{l|}{37}             & \multicolumn{1}{l|}{21.8}           & 11.5                              & \multicolumn{1}{l|}{20.8}           & \multicolumn{1}{l|}{38.6}           & 4.8                               \\ \hline
\textbf{Van-Tuning}             & \textbf{-}            & \multicolumn{1}{l|}{48.6}           & \multicolumn{1}{l|}{44.5}           & -3.7                              & \multicolumn{1}{l|}{18.3}           & \multicolumn{1}{l|}{50.2}           & -2.5                              \\ \hline
\textbf{Cor-RAIT}               & \textbf{-}            & \multicolumn{1}{l|}{41.3}           & \multicolumn{1}{l|}{18.3}           & 19.7                              & \multicolumn{1}{l|}{16.2}           & \multicolumn{1}{l|}{27.6}           & 4.7                               \\ \hline
\multirow{4}{*}{\textbf{CRaFT}} & \textbf{200}          & \multicolumn{1}{l|}{39}             & \multicolumn{1}{l|}{13.5}           & 23.2                              & \multicolumn{1}{l|}{16.5}           & \multicolumn{1}{l|}{24.9}           & 6.2                               \\ \cline{2-8} 
                                & \textbf{1000}         & \multicolumn{1}{l|}{38.5}           & \multicolumn{1}{l|}{12.9}           & 23.3                              & \multicolumn{1}{l|}{15.8}           & \multicolumn{1}{l|}{22.4}           & 6.5                               \\ \cline{2-8} 
                                & \textbf{3000}         & \multicolumn{1}{l|}{41.1}           & \multicolumn{1}{l|}{14.7}           & 23.9                              & \multicolumn{1}{l|}{18.1}           & \multicolumn{1}{l|}{28.2}           & 6.4                               \\ \cline{2-8} 
                                & \textbf{8000}         & \multicolumn{1}{l|}{40.2}           & \multicolumn{1}{l|}{14.4}           & 23.3                              & \multicolumn{1}{l|}{17}             & \multicolumn{1}{l|}{25}             & 6.7                               \\ \hline
\end{tabular}
{\fontsize{9pt}{11pt}\selectfont
\caption{Results of Reheasal Training in OEQA Task. ($\mathcal{M}_{0}$ is LLaMA2-7B-Chat)}
\label{table:ab_OEQA_rehearsal}}
\end{table}
\endgroup  % End the group

==> table/ab_OEQA_llama2.tex <==
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}

\begin{table}[t]
\centering
\label{table:ab_exp_OEQA}
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|c|ll|ll|}
\hline
\multicolumn{1}{|l|}{}  & \multicolumn{2}{c|}{\textbf{TriviaQA (ID)}}                             & \multicolumn{2}{c|}{\textbf{NQ (OOD)}}                                  \\ \hline
\textbf{Method}         & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS$\uparrow$}} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS$\uparrow$}} \\ \hline
\textbf{Cor-RAIT}       & \multicolumn{1}{l|}{18.32}          & 19.73                             & \multicolumn{1}{l|}{27.59}          & 4.71                              \\ \hline
\textbf{CRaFT w/o Flow} & \multicolumn{1}{l|}{20.45}          & 21.12                             & \multicolumn{1}{l|}{38.75}          & 5.15                              \\ \hline
\textbf{CRaFT w/o Cer}  & \multicolumn{1}{l|}{15.65}          & 20.11                             & \multicolumn{1}{l|}{22.13}          & 5.42                              \\ \hline
\textbf{CRaFT}          & \multicolumn{1}{l|}{12.93}         & 23.29                             & \multicolumn{1}{l|}{22.38}          & 6.54                              \\ \hline
\end{tabular}
}
\caption{Ablation Experiment Results in OEQA Task.}
\end{table}
\endgroup  % End the group

==> table/dataset_table.tex <==
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[h]
\centering
\begin{tabular}{|c|cc|cc|}
\hline
\textbf{}      & \multicolumn{2}{c|}{\textbf{MCQA}}        & \multicolumn{2}{c|}{\textbf{OEQA}}  \\ \hline
Train       & \multicolumn{1}{l|}{MMLU test}  & 14,079 & \multicolumn{1}{l|}{TriviaQA train} & 87,622 \\ \hline
ID Eval  & \multicolumn{1}{l|}{MMLU val}   & 1,540  & \multicolumn{1}{l|}{TriviaQA dev}   & 11,313 \\ \hline
OOD eval & \multicolumn{1}{l|}{ARC-c dev} & 1,172  & \multicolumn{1}{l|}{NQ dev}         & 3,610  \\ \hline
\end{tabular}
{\fontsize{9pt}{11pt}\selectfont
\caption{Details of the Datasets.}}
\label{table:dataset_details}
\end{table}
\endgroup

==> table/knowledge_state_query.tex <==
\begin{table*}[h!]
\begin{tabular}{|c|l|}
\hline
\centering
\textbf{Query Type}                                                                & \multicolumn{1}{c|}{\textbf{Instruction}}                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{Knowledge State Query} \\ \textbf{based on} \\ \textbf{TOKEN Probability}\end{tabular}    & \begin{tabular}[c]{@{}l@{}}There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\ 
\textbf{Question}: \{\textit{Question}\} \\
\textbf{A}. \{\textit{Context\_of\_A}\} \\
\textbf{B}. \{\textit{Context\_of\_B}\} \\
\textbf{C}. \{\textit{Context\_of\_C}\} \\
\textbf{D}. \{\textit{Context\_of\_D}\} \\
\textbf{Answer}:\textbf{\{\textit{Target\_Token}\}}(The Target Token takes on the values A, B, C, and D.)\end{tabular}                                                                                                                                                                                                                                                                                                    \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{Knowledge State Query} \\ \textbf{based on} \\ \textbf{Generation}\end{tabular} & \begin{tabular}[c]{@{}l@{}}There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\
\textbf{Question}: \{\textit{Question}\} \\
\textbf{A}. \{\textit{Context\_of\_A}\} \\
\textbf{B}. \{\textit{Context\_of\_B}\} \\
\textbf{C}. \{\textit{Context\_of\_C}\} \\
\textbf{D}. \{\textit{Context\_of\_D}\} \\
\textbf{Answer}:\end{tabular}                                                                                                                        \\ \hline                                                                                                                                                                                                                                                                                                                                         
\end{tabular}
\label{table:knowledege_state_query}
\caption{Prompt templates of the two type knowledge state query. The italic \{\textit{text}\} in curly braces represents variables that need to be replaced.}
\end{table*}

==> table/main_MCQA_ALL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[t]
\label{table:main_exp_MCQA}
\centering
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|c|c|lll|lll|}
\hline
\multicolumn{1}{|l|}{}                                                                  & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{MMLU (ID)}}                                                                       & \multicolumn{3}{c|}{\textbf{ARC-c (OOD)}}                                                                     \\ \hline
\textbf{Model}                                                                          & \textbf{Method}                & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama2-\\ 7B-\\Chat\end{tabular}}}     & \textbf{Init-Basic}            & \multicolumn{1}{l|}{\textbf{45.6}}  & \multicolumn{1}{l|}{52.8}           & 0                                 & \multicolumn{1}{l|}{53.9}           & \multicolumn{1}{l|}{46}             & 0                        \\ \cline{2-8} 
                                                                                        & \textbf{Init-Refuse}           & \multicolumn{1}{l|}{36.4}           & \multicolumn{1}{l|}{38.9}           & 3.9                               & \multicolumn{1}{l|}{44.4}           & \multicolumn{1}{l|}{\textbf{35.7}}  & 2.6                               \\ \cline{2-8} 
                                                                                        & \textbf{Van-Tuning}            & \multicolumn{1}{l|}{47}             & \multicolumn{1}{l|}{53.1}           & 1.2                               & \multicolumn{1}{l|}{54.5}           & \multicolumn{1}{l|}{45.5}           & 1.2                               \\ \cline{2-8} 
                                                                                        & \textbf{Cor-RAIT}              & \multicolumn{1}{l|}{44.5}           & \multicolumn{1}{l|}{39.6}           & 11.3                              & \multicolumn{1}{l|}{\textbf{55.8}}  & \multicolumn{1}{l|}{38.1}           & 11.1                              \\ \cline{2-8} 
                                                                                        & \textbf{CRaFT}                 & \multicolumn{1}{l|}{43.9}           & \multicolumn{1}{l|}{\textbf{36.4}}  & \textbf{12.5}                     & \multicolumn{1}{l|}{54.7}           & \multicolumn{1}{l|}{35.9}           & \textbf{12.6}                     \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3-\\ 8B-\\Instruct\end{tabular}}} & \textbf{Init-Basic}            & \multicolumn{1}{l|}{66.8}           & \multicolumn{1}{l|}{33.1}           & 0                                 & \multicolumn{1}{l|}{\textbf{80.6}}  & \multicolumn{1}{l|}{19.5}           & 0                                 \\ \cline{2-8} 
                                                                                        & \textbf{Init-Refuse}           & \multicolumn{1}{l|}{50}             & \multicolumn{1}{l|}{17}             & 15.7                              & \multicolumn{1}{l|}{65.3}           & \multicolumn{1}{l|}{14.4}           & 5.6                               \\ \cline{2-8} 
                                                                                        & \textbf{Van-Tuning}            & \multicolumn{1}{l|}{\textbf{69.5}}  & \multicolumn{1}{l|}{30.5}           & 8                                 & \multicolumn{1}{l|}{80.3}           & \multicolumn{1}{l|}{19.7}           & -1.3                              \\ \cline{2-8} 
                                                                                        & \textbf{Cor-RAIT}              & \multicolumn{1}{l|}{63.9}           & \multicolumn{1}{l|}{21.6}           & 20.4                              & \multicolumn{1}{l|}{79.4}           & \multicolumn{1}{l|}{16.2}           & 12.2                              \\ \cline{2-8} 
                                                                                        & \textbf{CRaFT}                 & \multicolumn{1}{l|}{53.3}           & \multicolumn{1}{l|}{\textbf{9.6}}   & \textbf{34}                       & \multicolumn{1}{l|}{74.1}           & \multicolumn{1}{l|}{\textbf{12.7}}  & \textbf{21.4}                     \\ \hline
\end{tabular}
}
\caption{Experimental Results in MCQA Task.}
\vspace{-10pt}
\end{table}
\endgroup  % End the group

==> table/main_OEQA_ALL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[t]
\label{table:main_exp_OEQA}
\centering
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|cc|lll|lll|}
\hline
\multicolumn{2}{|l|}{}                                                                                                               & \multicolumn{3}{c|}{\textbf{TriviaQA (ID)}}                                                                   & \multicolumn{3}{c|}{\textbf{NQ (OOD)}}                                                                        \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}}                                                                          & \textbf{Method}      & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama2-\\ 7B-\\Chat\end{tabular}}}}     & \textbf{Init-Basic}  & \multicolumn{1}{l|}{\textbf{54}}             & \multicolumn{1}{l|}{46}             & 0                                 & \multicolumn{1}{l|}{\textbf{29.3}}           & \multicolumn{1}{l|}{70.7}           & 0                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Init-Refuse} & \multicolumn{1}{l|}{37}             & \multicolumn{1}{l|}{21.7}           & 11.5                              & \multicolumn{1}{l|}{20.8}           & \multicolumn{1}{l|}{38.6}           & 4.8                               \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Van-Tuning}  & \multicolumn{1}{l|}{48.6}           & \multicolumn{1}{l|}{44.5}           & -3.7                              & \multicolumn{1}{l|}{18.3}           & \multicolumn{1}{l|}{50.2}           & -2.5                              \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Cor-RAIT}    & \multicolumn{1}{l|}{41.3}           & \multicolumn{1}{l|}{18.3}           & 19.7                              & \multicolumn{1}{l|}{16.2}           & \multicolumn{1}{l|}{27.6}           & 4.7                               \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{CRaFT}       & \multicolumn{1}{l|}{38.5}           & \multicolumn{1}{l|}{\textbf{12.9}}           & \textbf{23.3}                              & \multicolumn{1}{l|}{15.8}           & \multicolumn{1}{l|}{\textbf{22.4}}           & \textbf{6.5}                               \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3-\\ 8B-\\Instruct\end{tabular}}}} & \textbf{Init-Basic}  & \multicolumn{1}{l|}{\textbf{66.8}}           & \multicolumn{1}{l|}{33.2}           & 0                                 & \multicolumn{1}{l|}{\textbf{40.3}}           & \multicolumn{1}{l|}{59.7}           & 0                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Init-Refuse} & \multicolumn{1}{l|}{53.9}           & \multicolumn{1}{l|}{20.8}           & 12                                & \multicolumn{1}{l|}{31.1}           & \multicolumn{1}{l|}{38.6}           & \textbf{5}                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Van-Tuning}  & \multicolumn{1}{l|}{55}             & \multicolumn{1}{l|}{38.1}           & -21.9                             & \multicolumn{1}{l|}{21}             & \multicolumn{1}{l|}{48.5}           & -11.7                             \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Cor-RAIT}    & \multicolumn{1}{l|}{45.4}           & \multicolumn{1}{l|}{13.2}           & 18.8                              & \multicolumn{1}{l|}{17.2}           & \multicolumn{1}{l|}{\textbf{25.6}}           & -0.1                              \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{CRaFT}       & \multicolumn{1}{l|}{43.5}           & \multicolumn{1}{l|}{\textbf{10.9}}           & \textbf{21.5}                              & \multicolumn{1}{l|}{19}             & \multicolumn{1}{l|}{27.5}           & 0.4                               \\ \hline
\end{tabular}
}
\caption{Experimental Results in OEQA Task.}
\end{table}
\endgroup  % End the group

==> table/metric_example.tex <==
\begin{table}[h!]
\centering
\fontsize{9}{10}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{\diagbox{\( \mathcal{M}_0 \)}{\( \mathcal{M}_{t} \)}} & \multicolumn{3}{c|}{\( \mathcal{M}_1 \)} & \multicolumn{3}{c}{\( \mathcal{M}_2 \)} \\
\cline{2-7}
 & $\mathbf{N_C}$ & $\mathbf{N_W}$ & $\mathbf{N_R}$ & $\mathbf{N_C}$ & $\mathbf{N_W}$ & $\mathbf{N_R}$ \\
\hline
$\mathbf{N_C}$ & 30 & 10 & 10 & 25 & 10 & 15 \\
$\mathbf{N_W}$ & 0  & 10 & 40 & 5  & 5  & 40 \\
$\mathbf{N_R}$ & 0  & 0  & 0  & 0  & 0  & 0  \\
\hline
\end{tabular}}
\caption{State Changes for the Refined LLMs, \( \mathcal{M}_1 \) and \( \mathcal{M}_2 \), from the Initial LLM \( \mathcal{M}_0 \)}
\label{tab:data}
\end{table}


==> table/metric_shortness.tex <==
\begingroup
\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[h!]
\centering
{\fontsize{9pt}{10pt}\selectfont
\begin{tabular}{c|cc|cc}
\hline
Metric & $\mathcal{M}_1$ & $\mathcal{M}_2$ & $\mathcal{M}_3$ & $\mathcal{M}_4$ \\ \hline
$P_c\uparrow$ & 0.3 & 0.3 & 0.5 & 1 \\ 
$P_w\downarrow$ & 0.2 & 0.15 & 0 & 0 \\ 
$P_r$ & 0.5 & 0.55 & 0.5 & 0 \\ \hline
$S_{\text{honesty}}$ \cite{alignment_for_honesty} $\uparrow$ & (0.8) & (0.794) & (1) & (1) \\ 
TRUTHFUL \cite{cheng2024can} $\uparrow$ & (0.8) & (0.75) & 1 & 1 \\ 
rely \cite{rejection_improves} $\uparrow$ & (0.55) & (0.548) & 0.75 & 1 \\ 
R-Acc \cite{dont_hallucinate_abstain} $\uparrow$ & (0.8) & (0.778) & 1 & 1 \\ 
ER \cite{dont_hallucinate_abstain} $\uparrow$ & (0.3) & (0.25) & 0.5 & 1 \\ 
A-Acc  \cite{dont_hallucinate_abstain} $\uparrow$ & (0.8) & (0.75) & 1 & 1 \\ 
A-F1  \cite{dont_hallucinate_abstain} $\uparrow$ & (0.8) & (0.762) & 1 & 1 \\ 
AP \cite{R_Tuning} $\uparrow$ & — & — & (1) & (1) \\ \hline
THS (ours) $\uparrow$ & 0.1 & 0.15 & 0.5 & 1 \\ \hline
\end{tabular}
}
\caption{Comparison of refusal-aware metrics: The performance of constructed LLMs is \(\mathcal{M}_1 < \mathcal{M}_2 < \mathcal{M}_3 < \mathcal{M}_4\). However, existing metrics exhibit significant issues, as indicated by the numbers in (parentheses).}
\end{table}
\endgroup  % End the group

==> table/prompt_eval_REFUSE_MMLU.tex <==
\begin{table}[]
\centering

\begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
There is a single choice question about \{\textit{Task}\}. If you know the answer, please directly respond with the correct answer A, B, C, or D. If you do not know the answer, please respond with ``I don't know.".\\
\textbf{Question}:\{\textit{Question}\} \\
\textbf{A}. \{\textit{Content\_of\_A}\}\\
\textbf{B}. \{\textit{Content\_of\_B}\}\\
\textbf{C}. \{\textit{Content\_of\_C}\}\\
\textbf{D}. \{\textit{Content\_of\_D}\}\\
\textbf{Answer}: 
\end{tcolorbox}

\caption{The \textbf{REFUSE} Prompt Template for \textbf{Evaluation} on MMLU. The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
\label{table:prompt_eval_refuse_mmlu}

\end{table}


==> table/prompt_eval_REFUSE_TriviaQA.tex <==
% \begin{table}[]
% \caption{The \textit{refuse} prompt for evaluation on OEQA task. This prompt is applied to all methods EXCEPT \textit{Init-Basic}.}
% \label{table:prompt_eval_refuse_triviaqa}
% \centering
% \begin{tcolorbox}[arc=4mm]
% \begin{tabular}{p{\textwidth}c}

% Answer the following question, and if you don't know the answer, only reply with 'I don't know': \{question\} \\ 


% \end{tabular}
% \end{tcolorbox}
% \end{table}


\begin{table}[]
\centering

\begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
Answer the following question, and if you don't know the answer, only reply with ``I don't know": \{\textit{Question}\}
\end{tcolorbox}

\caption{The \textbf{REFUSE} Prompt Template for \textbf{Evaluation} on TriviaQA. The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
\label{table:prompt_eval_refuse_triviaqa}

\end{table}


==> table/prompt_kq_MMLU.tex <==
\begin{table}[]
\centering

\begin{tcolorbox}[title={In-Context Examples}, colback=white, coltitle=black, colbacktitle=white!0]
There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\
\textbf{Question}: \{\textit{Question1}\} \\
\textbf{A}. \{\textit{Content\_of\_A1}\}\\
\textbf{B}. \{\textit{Content\_of\_B1}\}\\
\textbf{C}. \{\textit{Content\_of\_C1}\}\\
\textbf{D}. \{\textit{Content\_of\_D1}\}\\
\textbf{Answer}: \{\textit{Answer1}\}\\
\\
There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\
\textbf{Question}: \{\textit{Question2}\} \\
\textbf{A}. \{\textit{Content\_of\_A2}\}\\
\textbf{B}. \{\textit{Content\_of\_B2}\}\\
\textbf{C}. \{\textit{Content\_of\_C2}\}\\
\textbf{D}. \{\textit{Content\_of\_D2}\}\\
\textbf{Answer}: \{\textit{Answer2}\}\\
\\
$\dots$
\\
There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\
\textbf{Question}: \{\textit{Question5}\} \\
\textbf{A}. \{\textit{Content\_of\_A5}\}\\
\textbf{B}. \{\textit{Content\_of\_B5}\}\\
\textbf{C}. \{\textit{Content\_of\_C5}\}\\
\textbf{D}. \{\textit{Content\_of\_D5}\}\\
\textbf{Answer}: \{\textit{Answer5}\}\\
\end{tcolorbox}

\begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
There is a single choice question about \{\textit{Task}\}. Answer the question by replying A, B, C or D.\\
\textbf{Question}: \{\textit{Question}\} \\
\textbf{A}. \{\textit{Content\_of\_A}\}\\
\textbf{B}. \{\textit{Content\_of\_B}\}\\
\textbf{C}. \{\textit{Content\_of\_C}\}\\
\textbf{D}. \{\textit{Content\_of\_D}\}\\
\textbf{Answer}:
\end{tcolorbox}

\caption{The Prompt Template for Knowledge State Query on MMLU. The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
\label{table:prompt_kq_MMLU}

\end{table}


==> table/prompt_kq_TriviaQA.tex <==

\begin{table}[]
    \centering
    
    \begin{tcolorbox}[title={In-Context Examples}, colback=white, coltitle=black, colbacktitle=white!0]
    Answer the following question as simple as possible.\\
    \textbf{Question}: \{\textit{Question1}\}\\
    \textbf{Answer}: \{\textit{Answer1}\}\\
    \\
    Answer the following question as simple as possible.\\
    \textbf{Question}: \{\textit{Question2}\}\\
    \textbf{Answer}: \{\textit{Answer2}\}\\
    \\
    Answer the following question as simple as possible.\\
    \textbf{Question}: \{\textit{Question3}\}\\
    \textbf{Answer}: \{\textit{Answer3}\}\\
    \end{tcolorbox}
    
    \begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
    Answer the following question as simple as possible.\\
    \textbf{Question}: \{\textit{Question}\}\\
    \textbf{Answer}: 
    \end{tcolorbox}
    
    \caption{The Prompt Template for Knowledge State Query on TriviaQA. The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
    \label{table:prompt_kq_triviaqa}
    
    \end{table}
    

==> table/prompt_train_REFUSE_MMLU.tex <==
\begin{table}[]
\centering

\begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
There is a single choice question about \{\textit{Task}\}. If you know the answer, please directly respond with the correct answer A, B, C, or D. If you do not know the answer, please respond with ``I don't know.".\\
\textbf{Question}:\{\textit{Question}\} \\
\textbf{A}. \{\textit{Content\_of\_A}\}\\
\textbf{B}. \{\textit{Content\_of\_B}\}\\
\textbf{C}. \{\textit{Content\_of\_C}\}\\
\textbf{D}. \{\textit{Content\_of\_D}\}\\
\textbf{Answer}: \{$Answer_{\text{rait}}$\} 
\end{tcolorbox}

\caption{The \textbf{REFUSE} Prompt Template for \textbf{Training} on MMLU. The The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
\label{table:prompt_training_refuse_mmlu}

\end{table}


==> table/prompt_train_REFUSE_TriviaQA.tex <==
% \begin{table}[]
% \caption{The \textit{refuse} prompt for training on triviaqa dataset train split. Loss is computed only on the underline \underline{texts}.}
% \label{table:prompt_train_refuse_triviaqa}
% \centering
% \begin{tcolorbox}[arc=4mm]
% \begin{tabular}{p{\textwidth}c}

% Answer the following question, and if you don't know the answer, only reply with 'I don't know': \{\textit{Question}\} \\ 
% \underline{\{answer_{\text{rait}}\}}


% \end{tabular}
% \end{tcolorbox}
% \end{table}

\begin{table}[]
\centering

\begin{tcolorbox}[title={Instruction}, colback=white, coltitle=black, colbacktitle=white!0]
Answer the following question, and if you don't know the answer, only reply with ``I don't know":\{\textit{Question}\}\\
\{$Answer_{\text{rait}}$\} 
\end{tcolorbox}

\caption{The \textbf{REFUSE} Prompt Template for \textbf{Training} on TriviaQA. The Italic \{\textit{text}\} in Curly Braces Represents Variables That Need To be Replaced.}
\label{table:prompt_training_refuse_triviaqa}

\end{table}

==> table/statistics_rehearsal.tex <==
\begingroup
\begin{table}[h!]
\setlength{\tabcolsep}{1mm}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{$n_{\text{rhs}}$} & \textbf{$n_{\mu < 0.5}$} & \textbf{$n_{\Delta \mu > 0}$} & \textbf{$n_{\mu < 0.5,\Delta \mu > 0}$} \\ \hline
\multirow{4}{*}{\textbf{MMLU}} & \textbf{200}   & 5175  & 4812  & 3318   \\ \cline{2-5}
                      & \textbf{500}   & 5175  & 5308  & 3252   \\ \cline{2-5}
                      & \textbf{1000} & 5175  & 4740  & 3571   \\ \cline{2-5}
                      & \textbf{1629}  & 5175  & 4389  & 3551   \\ \hline
\multirow{4}{*}{\textbf{TriviaQA}} & \textbf{200}   & 42457 & 9188  & 5102   \\ \cline{2-5}
                          & \textbf{1000} & 42457 & 9188  & 5034   \\ \cline{2-5}
                          & \textbf{3000} & 42457 & 9219  & 5061   \\ \cline{2-5}
                          & \textbf{8000} & 42457 & 11302 & 9553   \\ \hline
\end{tabular}
\caption{Comparison of Dataset Statistics across Different $n_{rhs}$ Values.}
\end{table}
\endgroup  % End the group

